Safe Stabilizing Control for Polygonal Robots in Dynamic Elliptical Environments

This paper addresses the challenge of safe navigation for rigid-body mobile robots in dynamic environments. We introduce an analytic approach to compute the distance between a polygon and an ellipse, and employ it to construct a control barrier function (CBF) for safe control synthesis. Existing CBF design methods for mobile robot obstacle avoidance usually assume point or circular robots, preventing their applicability to more realistic robot body geometries. Our work enables CBF designs that capture complex robot and obstacle shapes. We demonstrate the effectiveness of our approach in simulations highlighting real-time obstacle avoidance in constrained and dynamic environments for both mobile robots and multi-joint robot arms.

==> tex/Nonsmooth_Analysis.tex <==
% \section{Nonsmooth CBF Analysis}

% In this section, we adopt the theory of nonsmooth Control Barrier Functions (NCBFs) \cite{nonsmooth_cbf_1, polytopic_cbf} to ensure safety. This approach allows us to define safety constraints even when the collision-checking function is non-differentiable.

% We first argue that $\Phi$ is Lipschitz continuous and thus a candidate NCBF \cite[Definition 2]{nonsmooth_cbf_1}. 

==> tex/Polygon_SDF_BFGS.tex <==
\section{Collision-Checking Function Construction in Non-Convex Environments}
\label{sec: method}

In this section, we describe our approach to defining a collision-checking function for the system~\eqref{eq: dynamic} using an estimated environment Signed Distance Function (SDF) model $\tilde{\varphi}$ and a polygonal robot shape.

We define a polygon $\bfP(\bfq, \theta)$ for the robot state $\bfx = [\bfq, \theta]^\top$, representing the 2-dimensional physical domain associated with the robot state. The polygon is specified with $M$ edges $\{l_i\}_{i=1}^M$ and $M$ vertices $\{\bfp_i\}_{i=1}^M$.


We assume a Gaussian Processes (GP) estimation of the SDF environment, i.e. $\varphi(\bfq) \sim \mathcal{GP}(\tilde{\varphi}(\bfq),K_\varphi(\bfq,\bfq'))$, which can be obtained using \cite{gpis_lee}. 

Given the polygon $\bfP(\bfq, \theta)$ and the estimated continuously differentiable SDF $\tilde{\varphi}(\bfq)$, we compute a collision-checking function $\Phi: SE(2) \mapsto \bbR$ using the optimization program:

%
\begin{equation}
\label{eq: optimize_collision_function}
    \Phi(\bfq, \theta) := \min_{\bfy \in \bfP(\bfq, \theta)} \tilde{\varphi}(\bfy).
\end{equation}
%
Since the polygon is convex, we can restrict the search to the $M$ edges of the polygon, i.e, 
\begin{equation}
\label{eq: optimize_collision_edges}
    \Phi(\bfq, \theta) := \min_{\bfy \in \bfP(\bfq, \theta)} \tilde{\varphi}(\bfy) = \min_{i} \min_{\bfy \in l_i} \varphi(\bfy).
\end{equation}

However, due to the non-convexity of the SDF $\tilde{\varphi}$, it is not possible to obtain a closed-form expression for the optimizer in \eqref{eq: optimize_collision_edges}.
Therefore, we apply the Broyden–Fletcher–Goldfarb–Shanno (BFGS) \cite{NoceWrig06, Fletcher1988PracticalMO} algorithm to get the optimal solution. To ensure that the optimal value obtained from the BFGS algorithm is the global optimal solution, we apply the BFGS algorithm with $N = 10$ uniform  initial guesses on each edge $l_i$.

However, due to the non-convexity of the environmental SDF $\tilde{\varphi}$, the collision-checking function $\Phi$ may be non-differentiable, and the theory of CBF in Definition.~\ref{def: cbf} cannot be directly used.




% \subsection{SDF to CBF}

% This section shows that the constructed nonsmooth collision checking function $\Phi: SE(2) \mapsto \bbR$ is a valid candidate NCBF for the robotic system of a relative-degree one. 













==> tex/Quadrotor.tex <==
\section{Quadrotor Dynamics}
\label{sec: quad_eval}

In the following, we define the dynamics of a quadrotor as a control-affine system. A control-affine system can be represented as:
%
\begin{equation}
\dot{\mathbf{x}} = \mathbf{f}(\mathbf{x}) + \mathbf{g}(\mathbf{x})\mathbf{u}
\end{equation}
%
where $\mathbf{x}$ is the state vector, $\mathbf{u}$ is the control input, and $\mathbf{f}(\mathbf{x})$ and $\mathbf{g}(\mathbf{x})$ are vector fields. The state $\bfx$ is defined as a combination of position, velocity, rotation matrix, and angular velocity:
%
\begin{equation}
\mathbf{x} = [\mathbf{p}, \mathrm{R}, \mathbf{v}, \boldsymbol{\omega}]^\top \in \bbR^{18}
\end{equation}
%
where $\mathbf{p} \in \mathbb{R}^3$ is the position vector, $\mathrm{R} \in \mathbb{R}^{3\times 3}$ is the rotation matrix, $\mathbf{v} \in \mathbb{R}^3$ is the linear velocity vector, and $\boldsymbol{\omega} \in \mathbb{R}^3$ is the angular velocity vector.

The control input $\mathbf{u}$ is defined as:
%
\begin{equation}
\mathbf{u} = [\mathbf{F}, \boldsymbol{\tau}]^\top \in \bbR^4
\end{equation}
%
where $\mathbf{F} \in \mathbb{R}$ is the total thrust force along the $z$-axis, and $\boldsymbol{\tau} \in \mathbb{R}^3$ is the torque vector.

The dynamics of the quadrotor can be written as:

\begin{equation}
\begin{aligned}
\dot{\mathbf{p}} &= \mathbf{v} \\
\dot{\mathrm{R}} &= \mathrm{R} \mathrm{S}(\boldsymbol{\omega}) \\
\dot{\mathbf{v}} &= \frac{1}{m}(\mathrm{R} \mathbf{F}\mathbf{e}_3) - g\mathbf{e}_3 \\
\dot{\boldsymbol{\omega}} &= \mathrm{J}^{-1}(\boldsymbol{\tau} - \boldsymbol{\omega} \times \mathrm{J}\boldsymbol{\omega})
\end{aligned}
\end{equation}
%
where $m$ is the mass of the quadrotor, $\mathrm{J}$ is the inertia matrix, $g$ is the gravitational constant, $\mathbf{e}_3$ is the unit vector along the $z$-axis, $\times$ denotes the cross product between vectors, and $\mathrm{S}(\cdot)$ denotes the skew-symmetric matrix. Thus, we can define the components as follows:
%
\begin{equation}
\mathbf{f}(\mathbf{x}) =
\begin{bmatrix}
\mathbf{v} \\
\mathrm{vec}(\mathrm{R}\mathrm{S}(\boldsymbol{\omega}))\\
-g\mathbf{e}_3 \\
\mathrm{J}^{-1}(- \boldsymbol{\omega} \times \mathrm{J} \boldsymbol{\omega})
\end{bmatrix} \in \bbR^{18},
\mathbf{g}(\mathbf{x}) =
\begin{bmatrix}
\mathbf{0}_{3 \times 4} \\
\mathbf{0}_{9 \times 4} \\
\frac{1}{m}\mathbf{R} \mathbf{e}_3 \otimes \mathbf{e}_1^\top \\
\begin{bmatrix}
\mathbf{0}_{3 \times 1} & \mathrm{J}^{-1}
\end{bmatrix}
\end{bmatrix} \in \bbR^{18 \times 4},
\mathbf{u} =
\begin{bmatrix}
\bfF \\
\boldsymbol{\tau}
\end{bmatrix} \in \bbR^{4}. \notag
\end{equation}
%
where $\otimes$ denotes the Kronecker product, and $\mathbf{e}_1^\top = [1, 0, 0, 0]$. 



==> tex/Related_work.tex <==
\section{Related Work}
\label{sec: relate_work}

Obstacle avoidance, in both static and dynamic environments, has persistently been a central issue in robotics. Over the years, various algorithms and methodologies have been proposed to address this challenge.

At the planning level, several motion planning algorithms have been developed to provide a feasible path that ensures obstacle avoidance, including prominent approaches like $\textbf{A}^*$~\cite{A_star_planning},$\textbf{RRT}^*$~\cite{RRT_star}, and their variants~\cite{informed_rrt_star, neural_rrt_star}. However, those approaches typically assume the existence of a low-level tracking controller and may not be applicable in dynamic environments. and may not be applicable in dynamic environments. A significant contribution to the field was made by Khatib~\cite{potential-field}, who introduced artificial potential fields to enable collision avoidance during not only the motion planning stage but also the real-time control of a mobile robot. Later, Rimon and Koditschek \cite{navigation-function} developed navigation functions, a particular form of artificial potential functions. These functions strive to ensure collision avoidance and stabilization towards a goal configuration simultaneously. 
% Meanwhile, Fox \cite{Fox1997TheDW} introduced the dynamics window concept, an influential approach to obstacle avoidance that proactively filters out unsafe control actions. 
In recent years, research has delved into the domain of trajectory generation and optimization, with innovative algorithms proposed for quadrotor safe navigation~\cite{mellinger_snap_2011, zhou2019robust, tordesillas2019faster}. In parallel, the rise of learning-based approaches~\cite{michels2005high, pfeiffer2018reinforced, loquercio2021learning} has added a new direction to the field, utilizing machine learning to facilitate both planning and real-time obstacle avoidance. Despite their promise, these methods often face challenges in dynamic environments and in providing safety guarantees.


In the field of safe control synthesis, integrating control Lyapunov functions (CLFs) and control barrier functions (CBFs) into a quadratic program (QP) has proven to be a reliable and efficient strategy for formulating safe stabilizing controls across a wide array of robotic tasks~\cite{glotfelter2017nonsmooth, grandia_2021_legged, wang2017_aerial}. While CBF-based methodologies have been deployed for obstacle avoidance~\cite{srinivasan2020synthesis, Long_learningcbf_ral21, almubarak2022safety, dawson2022learning, abdi2023safe}, such strategies typically simplify the robot as a point or circle and assume static environments when constructing CBFs for control synthesis. Some recent advances have also explored the use of time-varying CBFs to facilitate safe control in dynamic environments~\cite{he2021rule, molnar2022safety, hamdipoor2023safe}. However, this concept has yet to be thoroughly investigated in the context of obstacle avoidance for rigid-body robots. For the safe autonomy of robot arms, Koptev \textit{et al}.\cite{Koptev2023_neural_joint_control} introduced a neural network approach to approximate the signed distance function of a robot arm and use it for safe reactive control in dynamical environment. 




Researchers~\cite{ding2022configurationaware} proposed a configuration-aware control approach for the robot arm by integrating geometric restrictions with Control Barrier Functions. 



Mostly related to our work, Thirugnanam \textit{et al}. \cite{discrete_polytope_cbf} introduced a discrete CBF constraint between polytopes and further incorporated the constraint in a model predictive control framework to enable safe navigation. The authors \cite{polytopic_cbf} also extended the formulation for continuous-time systems but the CBF computation between polytopes still remained numerical, requiring a duality-based formulation with non-smooth CBFs. 




\textbf{Contributions}: 1) We present an analytic distance formula in $SE(2)$ for elliptical and polygonal objects, enabling closed-form calculations for distance and its gradient. 2) We introduce a novel time-varying control barrier function tailored for robots described by one or multiple $SE(2)$ configurations based on the analytic distance. Its efficacy is validated through applications in ground robot navigation and multi-link robot arm demonstrations.













